Memory Organization for Energy-Efficient Learning and Inference in Digital Neuromorphic Accelerators

The energy efficiency of neuromorphic hardware is greatly affected by the energy of storing, accessing, and updating synaptic parameters. Various methods of memory organisation targeting energy-efficient digital accelerators have been investigated in the past, however, they do not completely encapsulate the energy costs at a system level. To address this shortcoming and to account for various overheads, we synthesize the controller and memory for different encoding schemes and extract the energy costs from these synthesized blocks. Additionally, we introduce functional encoding for structured connectivity such as the connectivity in convolutional layers. Functional encoding offers a 58% reduction in the energy to implement a backward pass and weight update in such layers compared to existing index-based solutions. We show that for a 2 layer spiking neural network trained to retain a spatio-temporal pattern, bitmap (PB-BMP) based organization can encode the sparser networks more efficiently. This form of encoding delivers a 1.37x improvement in energy efficiency coming at the cost of a 4% degradation in network retention accuracy as measured by the van Rossum distance.

==> graveyard.tex <==
% the gravyard of a very beautiful table

%\setlength{\tabcolsep}{3.5pt}

%\begin{table}[!t]
%\centering
%\begin{tabular}{ccccccc}
%\toprule
% &  &\multicolumn{3}{c}{Gradient Bits }&  \\
%$b_w$ & 8 & 9 & 10 & 11 & 12\\
%\midrule
%2 & 3263 \textit{$\pm147$} & 3547 \textit{$\pm206$} & 4174 \textit{$\pm77$} & 4792 \textit{$\pm198$} & 5523 \textit{$\pm133$}\\
% & (9826)  & (9910)  & (9984)  & (9964)  & (9977) \\
%3 & 3238 \textit{$\pm120$} & 3704 \textit{$\pm167$} & 4349 \textit{$\pm126$} & 4862 \textit{$\pm150$} & 5433 \textit{$\pm158$}\\
% & (9774)  & (9976)  & (9986)  & (9983)  & (9963) \\
%4 & 3433 \textit{$\pm149$} & 3824 \textit{$\pm164$} & 4355 \textit{$\pm184$} & 4954 \textit{$\pm157$} & 5282 \textit{$\pm139$}\\
% & (9962)  & (9987)  & (9982)  & (9979)  & (9981) \\
%5 & 3387 \textit{$\pm194$} & 3814 \textit{$\pm136$} & 4268 \textit{$\pm190$} & 4756 \textit{$\pm118$} & 5305 \textit{$\pm54$}\\
% & (9954)  & (9982)  & (9989)  & (9974)  & (9986) \\
%6 & 3340 \textit{$\pm88$} & 3803 \textit{$\pm104$} & 4183 \textit{$\pm95$} & 4779 \textit{$\pm96$} & 5217 \textit{$\pm156$}\\
% & (9819)  & (9988)  & (9987)  & (9991)  & (9990) \\
%\bottomrule
%\end{tabular}
%\caption{Best van Rossum distance (with standard deviation) after training for different weight and gradient bit levels (error and membrane computation kept constant at 12 bits). Numbers averaged over 5 runs. Average total of epochs needed to reach best distance given brackets.}
%\label{tab:table_grads_weight}

%\end{table}


%the interplay of all of them. The Energy consumption is building upon a forward and backward pass given a experimentally obtained sparsity level of a quantization configuration. The symbols again indicate the used data structure. \cs{We can observe an efficient frontier which trades off energy versus van Rossum distance for the learning of our spatio-temporal pattern.}


% \cs{Overall the configuration of 5 bits for weights, 12 bits for membrane computations and error and 8 bits for gradients achieved the best temporal pattern retention with a van Rossum distance of 3014.49. Generally more bits available for the membrane potential computation help the optimization goal of a smaller van Rossum distance.}



%\begin{figure}[!t]
%\centering
%\includegraphics[width=3.5in]{figures/2888.png}
%\caption{Energy for Performance 2888}
%\label{fig_sparsity}
%\end{figure}

%\begin{figure}[!t]
%\centering
%\includegraphics[width=3.5in]{figures/6888.png}
%\caption{Energy for Performance 6888}
%\label{fig_sparsity}
%\end{figure}






%%% Sparsity Leakage Contribution Convolutional


% Figure \ref{fig_vr_meaning} illustrates the meaning of the of van Rossum distance in our experiments for a sample configuration (no quantization and learning rate of $0.001$). Our target was a spatio-temporal pattern similiar to the smiley face which emerges after 6400 epochs. The four different spatio-temporal patterns shown correspond to four different levels of van Rossum distances. The first (from the left) represent random temproal and spatial spikes and has a van Rossum distance of $6590.25$, meanwhile the next three patterns have van Rossums distances of $4771.20$, $3927.91$ and $3023.19$ respectivly.






%\begin{figure}[!t]
%\centering
%\includegraphics[width=3.5in]{figures/sparsity.png}
%\caption{Energy Quant Tradeoffs}
%\label{fig_sparsity}
%\end{figure}


%\begin{figure}[!t]
%\centering
%\includegraphics[width=3.5in]{figures/fc_sweep.png}
%\caption{Activity}
%\label{fig_sparsity}
%\end{figure}


% Table \ref{tab:table_grads_weight} tabulates the effect of forward we the best van Rossum distance of our SNN setup after training for 10000 epochs for various quantization setups. The error and membrane computations levels were kept constant at 12bits for Table \ref{tab:table_grads_weight} meanwhile weights and gradient quantization levels varied. 

% As a learning rule we used SuperSpike as presented in~\cite{neftci2019surrogate} with a normalized negative part of a fast sigmoid of the membrane potential as a surrogate gradient.
%  We set a fixed $\alpha = .75$ (synaptic decay), $\beta = .875$ (membrane decay) and $\gamma = 0$ for the neuron dynamics. The fixed $\alpha$ and $\beta$ represent shifts on a hardware level and hence simplify the computation of the decay dynamics. The threshold for our LIF neurons was set at $.9$ (to be reachable in quantized computations) and reset of the neuron was done by subtraction of $1$ (e.g. $\delta = 1$) from the membrane potential, since the reset decay constant is set to zero and hence accounting for a small refractory period. We chose stochastic gradient descent as an optimizer and ran our experiments with an learning rate of $1$. The gradient was normalized with its largest absolute value during the quantization step.
%\eon{1? are you sure? A stored weight would be wiped if this were the case. I think the following step may be consfusing (its an implementation technicality). The Va Rossum figure is nice but seems out of context here.}
% The learning rate was applied in the gradient quantizaton step and not by the optimizer. The weights were initialized according to the methodology in~\cite{wu2018training}, which is uniform between two bounds depended on the quantization and layer size. 


%For a fully-connected layer with $8$ bits of weight quantization, $784$ inputs, and $128$ outputs, PB-CSR requires $2.31$ times as much energy for the forward pass and $1.34$ times as much energy for the backward pass as PB-BMP at a density of $.5$, while requiring $2.41$ times as much energy for the forward pass and $1.55$ times as much energy for the backward pass as PB-BMP at a density of 1.


%\%section*{Acknowledgment}
%Placeholder due to double blind review process.

%The authors would like to thank the CVRL group and Prof Hu for granting access to their GPU systems.

%\begin{thebibliography}{1}

%\bibitem{IEEEhowto:kopka}
%H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

%\end{thebibliography}

 %Thus, the how that shows which data structure performs best under difference conditions of sparsity and leakage contribution. The symbol indicates the best data structure for a given configuration and the color shows the logarithm of the consumed energy for a fully connected forward and backward pass. \cs{We can see a clear split between Crossbar and PB-CSR, corssbar naturally works best under conditions of density whereas PB-CSR work well given sparsity. Further on, energy consumption spikes for extreme values of leakage contribution.}

% As Fig. \ref{fig_fc} shows, pointer-based implementations perform comparatively well when compared to a crossbar in sparse scenarios. The crossbar needs to read a set number of memory locations which is independent of the sparsity, while the PB-CSR and PB-BMP approaches can leverage sparsity to reduce both the memory size, which means fewer reads are required in the forward and backward passes. This means that less energy is required overall, which leads to the shape shown. As Fig. \ref{fig_sparsity} shows, the PB-CSR and crossbar approaches are the most energy-efficient at very high and very low sparsities, while PB-BMP is the most efficient everywhere else. Both PB-BMP and PB-CSR store a pointer table and a weight table, but PB-CSR has a larger weight table due to the storage of post-synaptic connections while PB-BMP stores a binary adjacency table. The weight table is sparsity-dependent while the adjacency and pointer tables are sparsity-independent, so PB-CSR benefits more from high sparsity than PB-BMP, which is why PB-CSR is more efficient for very low densities.

% Figure \ref{fig_conv} shows the relative effectiveness of different access methods for a convolutional layer. In the forward pass, the approaches each require a similar amount of energy, with the increased reads in the pointer-based methods being offset by more additions required to compute the connectivity in the Func-RowCol approach. In the backward pass, however, PB-CSR suffers from a large amount of overhead required to find the connectivity. PB-BMP also suffers from some overhead in the backward pass, while the functional row-column remains largely the same, with an increased number of subtractions being offset by a decreased number of additions. 


%\sj{Recent advances in neuromorphic engineering have shown remarkable results in using spiking neural network for a range of tasks such as (robotics, blah, blah, blah). Critically, many of these tasks require that a network be able to update its parameters after training, put in something about continual “life-long” learning.}

%systems  Spiking Neural Networks are a biologically inspired approach, which could bring the power of DNNs to low power devices, given their theoretical efficiency for learning. 

% However, state of the art results usually come at the cost of energy, due to the extensive use of computationally expensive multiply and accumulate operations in neural networks (mostly done on GPUs) during inference and training. Researchers have addressed the issue of DNNs power consumption in several ways; 
% Also add in an introduction of how SNNs work - spikes come in, look up weights, do the MAC - followed by something that generates subsequent spikes


%-----
%all the diffiuclties with implemeting SNNs
%Many way SNN, most important things -> accessing weights during inference and training 

%------
%- Neural Networks import DNNs -> Spiking Neural %Networks important\usepackage{}
%- Energy efficient learning inspired by biology
% Deep neural networks (DNNs) have achieved state of the art performance in a range of fields like computer vision~\cite{krizhevsky2012imagenet}, natural language processing~\cite{deng2013new,glorot2011domain}, computer-aided diagnosis~\cite{cheng2016computer}, and abstract strategic planning~\cite{silver2016mastering}. While DNNs are loosely inspired by the biological brain,

%access timeinvestigated the efficiency storing sparse synaptic connectivity and weights using digital memory organized to accommodate different data structures such as compressed sparse row (CSR), index-based run-length encoded (RLE), and index-based bitmap (BMP). Building on this,~\cite{} argued that just analyzing storage efficiency did not sufficiently encompass all costs encountered during on-chip learning and introduced a metric that included memory access costs as well as storage-costs to better encapsulate the energy impact of different representation formats
% This is explored in~\cite{} One crucial step in \ac{STDP}, the ``reverse'' look-up, entails determining all pre-synaptic neurons connected to a given post-synaptic neuron.  \eon{Explain the backward table look-up problem, }
% In this paragraph - we talk about the hardware systems and the challenges that are involved in implementing these hardware systems. Specifically start talking about how memory is a major component of neuromorphic systems. Talk about how there's memory for each weight - and the connectivity has high-fanout. Talk about how this can dominate the energy (here reference other papers) - even if it doesn't dominate - it can definitely limit scalability.

% 1) Spiking neural networks
% 2) LIF neurons
% 3) memory accesses dominate in terms of energy, and memory area is also important.
% 4) On chip learning is important, and the next frontier - many people concentrate on inference on chip - learning in a data -center - many applications such as mobile systems , robotics, "life-long-learning" - things require this.
% However, efficient implementations of different network topologies Another challenge is that hardware implementations face difficulties connecting neurons and transmitting information, a problem already analyzed by \cite{sakai2019dropout}. From a perspective focusing on energy, it becomes evident that SNNs come with the advantage of theoretically being very energy efficient due to the use of spikes [?]. One thing implementation of SNNs share so far is that energy-wise it is costly to access weights during training and inference.
% Recent advances in the development of learning algorithms that leverage spiking networks have resulted in SNNs that perform competitively with their rate-based counterparts~\cite{zenke2018superspike,shrestha2018slayer}. 


%%The development of energy-efficient SNNs faces significant challenges. One primary challenge is that the activation functions are spike-based and hence, standard methods for learning such a backpropagation do not work. Nevertheless, several researchers already addressed this issue, most notably are approaches which work with surrogate gradients \cite{zenke2018superspike, shrestha2018slayer}.




%-----
%Many people Joshi, Bruno optimized access times storage efficient rather optimizing for energy.
%this paper energy efficient training inferenec of digital implementation of spiking NN
%-----% ~\cite{} showed that synapse memory structure indeed matters, they proposed a efficient synapse memory structure, implemented it in CMOS and showed that using it yields 200x speedup for SNNs compared to running them on normal CPUs.


%spiking neural network
%% Emre: remove following if not needed.
% SG learning is currently the state-of-the-art on spike-based classification benchmark tasks \cite{Shrestha_Orchard18_slayspik,Bellec_etal19_biolinsp,Kaiser_etal18_synaplas}.

%, to determine the energy for different  for different memory sizes precisely quantifying the tradeoff between . THEN TALK MORE ABOUT WHAT WE DO IN THIS PAPER.

% various tradeoffs associated with this memory.  Previous works on energy optimisation for SNNs have focused primarily on access time. For example, \cite{} anaylzed the use of a range of storage schemes from crossbar arrays to pointer-based lookups given varying levels of densities and elaborated on the tradeoffs of each method given cost and efficiency. Both studies showed tradeoffs for their memory organisation methods based on access time and storage efficiency, but not for overall energy consumption. This paper will examine the tradeoffs of accuracy and energy consumption for quantized SNNs for training and inference and hence facilitating better design of hardware and algorithms with low power consumption.  

%\section{Related Work}


%------
%see wage, here for convencie some results -> but for %further details see.
%------


%Quick Reference to Moons and QNNs




% \sj{describe the function equation here}



% in comparison to  followed by  an example, we use a convolutional pattern to demonstrate the advantage of using  the performance This paper introduces a functional approach to better compress  on the consideration that in a convolutional layer a synaptic connections follow a repeated pattern. 
% Shown in~\ref{fig:forwardfunc}.
%Different Weight Access scheme(?) Run Length Encodeing, (Bruno) -> access efficiency/storage efficiency


%\cs{suggestion: The function $\Theta$ is the step function, \emph{i.e.} $S_i[n]=1$ when $U_i[n]=0$. Actually not really sure, I'd say we need to introduce the threshold here? + if we want to do the when 0 spike thing, then we need to subtract the threshold from the mem}

%\begin{equation}\label{eq:loss}
%\frac{\partial}{\partial W_{ij}} \mathcal{L} = 
%\frac{\partial}{\partial S_{i}}\mathcal{L}
%\frac{\partial}{\partial U_{i}}S_i  
%\frac{\partial}{\partial W_{ij}}U_i
%\end{equation}
%%We discuss below the calculation of each of the three factors in the equation above from right to left.
%The rightmost factor 
%%$\frac{\partial}{\partial W_{ij}}U_i$  
%describes the change of the membrane potential with respect to the weight $W_{ij}$.
%This term is equal to $P_j[n] - \frac{\partial}{\partial W_{ij}}R_i[n]$ for the neuron defined by \eqref{eq:lif_equations}. To simplify this expression, we ignore the dependence of $R$ on the past spiking activity of the neuron, as in~\cite{Zenke_Ganguli17_supesupe}. 


% Let's talk about this in the experiments section \subsection{Energy Measurement Techniques}
% How much energy does weight access take, forward pass, backward pass, derivative computation(?), weight update(?)

 %Thus, $b_w$ can be written as 
    % $q(w) =\sigma(b_w) \cdot \text{round} \left[\frac{w}{ \sigma(b_w)}\right] $
    
    
%though the PB-BMP does not have extremely efficient backward pass, the more compact storage %quantization on the energy different datastructure consum for accessing weights. \cs{Describe results of quant energy trade off for fc and conv}


%to support arbitrary sparse connectivity.  The crossbar method stores synaptic connectivity in a dense matrix form, where every connection between a pre- and post-synaptic neuron has a place in a weight table even if this weight is zero. The crossbar method is appropriate for fully connected dense layers. The PB-CSR only stores weights of connection which actually exist by using start and end pointers to compress the fully dense connection matrix. In case of very sparse connectivity the pointer-base compressed sparse row data structure offers a more memory efficient way to access weights compared to the crossbar. A mix of the crossbar and PB-CSR method is the pointer-based bitmap, which builds upon a weight pointer table, weight table and binary adjacency table to store and access weight. PB-BMP utilizes the binary adjacency table to store the information of whether a connection exists or not. If a connection exists, it accesses the next weight through the next pointer in the pointer table.

% since there is no level of indirection involved, it also removes the need for a separate memory structure which might incur leakage power costs despite this also Our functional approach builds on the consideration that in a convolutional layer a synaptic connections follow a repeated pattern. During a forward pass, memory accesses can be reduced by directly accessing weights without looking them up through pointer tables or 
% \eon{this also reduces the memory required in the pointer table,no?} %Different Weight Access scheme(?) Run Length Encodeing, (Bruno) -> access efficiency/storage efficiency
